Under the Sand: Navigation and Localization of a Micro Aerial Vehicle for Landmine Detection with Ground Penetrating Synthetic Aperture Radar

Ground penetrating radar mounted on micro aerial vehicle (MAV) is a promising tool to assist humanitarian landmine clearance. However, the quality of synthetic aperture radar images depends on accurate and precise motion estimation of the radar antennas as well as generating informative viewpoints with the MAV. This paper presents a complete and automatic airborne ground-penetrating synthetic aperture radar (GPSAR) system. The system consists of a spatially calibrated and temporally synchronized industrial grade sensor suite that enables navigation above ground level, radar imaging, and optical imaging. A custom mission planning framework allows generation and automatic execution of stripmap and circular (GPSAR) trajectories controlled above ground level as well as aerial imaging survey flights. A factor graph based state estimator fuses measurements from dual receiver real-time kinematic (RTK) global navigation satellite system (GNSS) and inertial measurement unit (IMU) to obtain precise, high rate platform positions and orientations. Ground truth experiments showed sensor timing as accurate as 0.8 us and as precise as 0.1 us with localization rates of 1 kHz. The dual position factor formulation improves online localization accuracy up to 40% and batch localization accuracy up to 59% compared to a single position factor with uncertain heading initialization. Our field trials validated a localization accuracy and precision that enables coherent radar measurement addition and detection of radar targets buried in sand. This validates the potential as an aerial landmine detection system.

==> reviews/responses.tex <==
We would like the thank all reviewers and the editor for their careful reviews of our manuscript, and their constructive comments. We have revised our submission in response to reviewer comments and we believe that the revised paper is clearer. We have appended a copy of the revised paper to the end of this document with major changes from the previous version highlighted in \textcolor{blue}{blue}. There were numerous minor changes throughout the paper, but we tried to limit the amount of blue text to indicate only the more significant revisions.

\section{Common Responses}
Firstly, we would like to address comments made by multiple reviewers, and more general revisions to the manuscript. We address more specific comments and provide responses for each reviewer in the following sections.

More significant changes in the revised manuscript are:
\begin{itemize}
    \item 
\end{itemize}

\section{Reviewer 1}
Thank you for the positive feedback and for identifying some key areas for improvement. 


==> reviews/review1.tex <==
Reviewing: 1

Additional Questions:
What is this paper about?: The subject of the paper is the configuration and performance of an airborne sensor suite that provides good pose information about the vehicle and the sensors aboard to enable good localization of the overall system and specifically, provide assessment of buried objects. Specific attention is paid to calibration of the relative geometry of the physical system and the timing of the information from a variety of sensors.

Select the most appropriate description of manuscript: Systems Article

What about this work is original, novel, and unique?: This work combines and builds upon earlier results in a unique way. While primarily a system integration, there are specific areas, such as time synchronization where the authors have taken a comprehensive look at a systemic issue.

Why is this paper significant and is this enough to warrant publication?: It's rare to have a full system paper that also discusses core  and critical technologies in depth. Yes, the papper warrants publication.

Does the paper describe its underlying theoretical principles?: Generally yes. Navigation section reviews the tracking controller, altitude estimation, and trajectory generation. Similarly, the time synchronization for the tracking by breaking the task down into three parts. The theoretical principles are primarily done by reference - Kalman filters, factor graph, etc by reference.

Are these principles well explained and correctly applied?: Yes. In addition to providing an excellent background and prior work, this work builds on those efforts to show how careful attention to very specific problems of pose estimation, timing synchronization are addressed.

Does the paper provide compelling experimental evidence?: There are three specific experiments shown and the experiments are good, but in at least one case, limited. It would have been useful to have a fully integrated GNSS system but there may have been practical reasons including cost and time. There is one part in that by using the Vicon system it doesn’t really reflect actual GPS data and since everything from timing information to GPS data is done through a relative geometry, I suspect integrating this will matter.

Are the experiments well conceived, sufficient in scope, and statistically significant?: There were three types of experiments that were carried out. However, there is no indication that the experiments were repeated multiple times to see what, if any, differences there might be. In general for field robotics, there is a tendency to run experiments until one works and then publish the results. So rather than running 10 experiments and publishing when one works, to truly confirm results, 10 experiments could be run and perhaps 1 may fail. That would be a better outcome than one or two experiments. But the paper makes clear what the experiments were and the results from all of them.

Does the paper contain adequate technical detail to confirm its correctness?: Yes, there is a solid consideration of choices made and the details of the system, testing, and experiments.

Does the paper report on what was learned?: The conclusion reports on the overall success of the approach but also what improvements and changes they would make with further testing and experiments.

Is the paper logically organized?: Organization is clear and direct and understandable.

Is the writing understandable? Are there noteworthy grammatical problems?: The writing is well edited and no noteworthy grammatical issues were observed during multiple readings.

Does the abstract succinctly summarize the main ideas and results of the work?: Yes, key ideas in timing and calibration, mission framework (something often overlooked in these studies) are nicely captured in the abstract.

Does the introduction provide motivation and overview of the work?: Motivation of saving lives, improving field results from airborne system, and improvements at the system level are very good overview of the subject and purpose of the work.

Are the figures informative and clear with proper labeling?: Yes, the figures are understandable, and clearly referenced in the text.

Are the captions explanatory of the figure content?: The captions are clear and complete sentences - not fragments or obscure.

Does the summary/conclusion meaningfully describe the contribution and result?: Yes it does.

Are adequate citations made for prior work or controversial statements?: Generally, yes and are notable in breadth.

Is the bibliography complete?: Many good references though I didn’t see reference to the airborne work by Singh, Zhang, and
Scherer at CMU who have been building fully autonomous airborne systems at CMU for more than a decade.


==> reviews/review2.tex <==
Reviewing: 2

Comments:
The paper clearly represents a tremendous amount of work building a non-trivial real-world system that operates in the field. The only question the reviewer had was regarding the note that "in practice every sensor will introduce some small uncompensated delay" - very good of the authors to mention this - is there any concern that these small delays, together, could compromise performance? (Likely not?)

Additional Questions:
What is this paper about?: The paper describes the design, development, implementation, and testing of a novel UAV-mounted ground-penetrating synthetic aperture radar (GPSAR) system. The target use case is detection of buried landmines. Extensive field trials are presented that demonstrate the potential of the system to detected mines buried in sand.

Select the most appropriate description of manuscript: Systems Article

What about this work is original, novel, and unique?: The article presents a unique, low cost and lightweight GPSAR system that can be carried by a small COTS UAV (the DJI M600). To the best of the reviewer's knowledge, this is the first such system that achieves the required positioning accuracy (as a result of careful design and calibration) to produce usable SAR images for this type of detection task.

Why is this paper significant and is this enough to warrant publication?: In addition to being well written, the paper is an outstanding example of precision robotics design and implementation to solve a challenging problem. The level of technical detail is excellent and the task itself is important (given the number of deaths caused by landmines each year).

Does the paper describe its underlying theoretical principles?: Yes, the underlying theoretical principles are clearly described and discussed. In particular, Section 3 provides a concise and valuable overview of SAR imaging, while Section 6 details the (novel) time synchronization method that is applied (to achieve the necessary positioning accuracy).

Are these principles well explained and correctly applied?: The principles are very well explained and correctly applied.

Does the paper provide compelling experimental evidence?: The paper provides experimental results from real-world field trials with the UAV platform.

Are the experiments well conceived, sufficient in scope, and statistically significant?: The experiments are well conceived and developed and sufficient in scope. Proper ground truthing and evaluation is also considered, which is very important. The reviewer commends the authors for their efforts in this area. Also, the study of buried object detection is well explained.

Does the paper contain adequate technical detail to confirm its correctness?: The technical content of the paper is excellent and more than sufficient to determine correctness. It would be useful in Section 4.1 to define the notation used for the left/right subscripts on the homogeneous transformation matrices.

Does the paper report on what was learned?: The paper reports on what was learned incrementally throughout the various sections, and also provides a summary of important points at the end.

Is the paper logically organized?: The paper is logically organized and flows well.

Is the writing understandable? Are there noteworthy grammatical problems?: The writing is clear and concise throughout; the reviewer did not find any substantial grammatical errors.

Does the abstract succinctly summarize the main ideas and results of the work?: The abstract clearly and succinctly summarizes the main contributions of the paper and provides an overview of the system's localization performance.

Does the introduction provide motivation and overview of the work?: The introduction provides a clear overview and also a compelling motivation (statistics on landmine casualties).

Are the figures informative and clear with proper labeling?: In general, yes. Figure 1 could perhaps be augmented with additional labels (beyond just (a) and (b)). In Figure 3a, it is very difficult to see the frame references and text labels - could the background image perhaps be 'faded' to make the labels more legible? (e.g., like Figure 8)

Are the captions explanatory of the figure content?: The captions do a good job of explaining the figures.

Does the summary/conclusion meaningfully describe the contribution and result?: The conclusion succinctly describes the contributions of the paper and the experimental results obtained. It also lays out several directions for future work.

Are adequate citations made for prior work or controversial statements?: The authors have done an excellent job of citing and summarizing prior work in this area and situating their contributions.

Is the bibliography complete?: The bibliography is complete.

==> reviews/review3.tex <==
Reviewing: 3

Comments:
This article presents an accurate localization system to improve the quality of SAR images retrieved from an airborne GPSAR system. This is an interesting topic but from the analysis of the results it is not clear that this yields a noticeable improvement in the SAR images. It is obvious that RTK GNSS positioning outperforms DJI positioning, but the results do not show an improvement in SAR image quality when the proposed localization system is used instead of RTK GNSS (i.e, DJI+RTK).

Although the authors state that DJI+RTK solution requires a known transformation to the base frame, this transformation can be indeed obtained and, therefore, it is not a proper reason to justify the need of the proposed localization system.

Therefore, the authors should either find a proper reason or a situation where the proposed localization system is essential to retrieve good subsurface SAR images or find another application where this kind of localization system is essential (e.g., a higher frequency radar application).

Furthermore, results in a non-smooth scenario must also be included as the results shown in the manuscript correspond only to smooth areas. It is essential to know how the proposed system works in a non-smooth terrain.

Also concerning the results section, results in section 8.3. must include those corresponding to DJI+RTK system in order to compare both positioning systems when buried object detection is performed.

There are also several further issues that I believe the authors should address.
1) I would shorten the title to “Navigation and Localization of a Small Unmanned Aerial Vehicle for Landmine Detection” as the article focuses mostly on the localization of the UAV.
2) In the Introduction and Related Work sections, the state-of-the art in landmine detection should be updated as there are a considerable number of new publications in this field (besides those of the authors).
3) Section 4.2. “Mission Overview” should be considerably shortened or removed as it describes typical mission planning strategies and programs.
4) The 6 cm shift in the location of the buried target (Fig. 22) is too large for this scenario and frequency range, could you find a proper reason for this shift?
5) Reprojection is used sometimes instead of backprojection (I would recommend using backprojection always).
6) The article is too long, and it contains some paragraphs or figures that do not add valuable information (e.g., Fig. 21a must be removed).


Additional Questions:
What is this paper about?: This article presents an accurate localization system to improve the quality of SAR images retrieved from an airborne GPSAR system.

Select the most appropriate description of manuscript: Regular Article

What about this work is original, novel, and unique?: They proposed a novel localization system for the UAV to improve the quality of the SAR images, but this improvement is not clearly shown in the results.

Why is this paper significant and is this enough to warrant publication?: It should be improved to warrant publication.

Does the paper describe its underlying theoretical principles?: Yes.

Are these principles well explained and correctly applied?: Yes.

Does the paper provide compelling experimental evidence?: No, more experiments should be included dealing with non-smooth terrains.

Are the experiments well conceived, sufficient in scope, and statistically significant?: No, as aforementioned, all the scenarios are flat terrains.

Does the paper contain adequate technical detail to confirm its correctness?: Mostly yes.

Does the paper report on what was learned?: Yes.

Is the paper logically organized?: Yes, but it is too long.

Is the writing understandable? Are there noteworthy grammatical problems?: Yes, it is understandable and there are no major mistakes.

Does the abstract succinctly summarize the main ideas and results of the work?: Yes.

Does the introduction provide motivation and overview of the work?: Yes, although the state-of-the-art should be a little bit updated.

Are the figures informative and clear with proper labeling?: Yes, although some of them do not add valuable information.

Are the captions explanatory of the figure content?: Yes.

Does the summary/conclusion meaningfully describe the contribution and result?: Mostly yes, but it is again not clear the improvement in the SAR images (that is, the need for the accuracy of the proposed localization system).

Are adequate citations made for prior work or controversial statements?: Yes.

Is the bibliography complete?: Mostly yes, but it should be a little bit updated
